Self-Repellent Random Walks on General Graphs -- Achieving Minimal Sampling Variance via Nonlinear Markov Chains

We consider random walks on discrete state spaces, such as general undirected graphs, where the random walkers are designed to approximate a target quantity over the network topology via sampling and neighborhood exploration in the form of Markov chain Monte Carlo (MCMC) procedures. Given any Markov chain corresponding to a target probability distribution, we design a self-repellent random walk (SRRW) which is less likely to transition to nodes that were highly visited in the past, and more likely to transition to seldom visited nodes. For a class of SRRWs parameterized by a positive real {\alpha}, we prove that the empirical distribution of the process converges almost surely to the the target (stationary) distribution of the underlying Markov chain kernel. We then provide a central limit theorem and derive the exact form of the arising asymptotic co-variance matrix, which allows us to show that the SRRW with a stronger repellence (larger {\alpha}) always achieves a smaller asymptotic covariance, in the sense of Loewner ordering of co-variance matrices. Especially for SRRW-driven MCMC algorithms, we show that the decrease in the asymptotic sampling variance is of the order O(1/{\alpha}), eventually going down to zero. Finally, we provide numerical simulations complimentary to our theoretical results, also empirically testing a version of SRRW with {\alpha} increasing in time to combine the benefits of smaller asymptotic variance due to large {\alpha}, with empirically observed faster mixing properties of SRRW with smaller {\alpha}.

==> Sections/Acknowledgements.tex <==
% Acknowledgements and Disclosure of Funding should go at the end, before appendices and references

All acknowledgements go at the end of the paper before appendices and references.
Moreover, you are required to declare funding (financial activities supporting the
submitted work) and competing interests (related financial activities outside the submitted work).
More information about this disclosure can be found on the JMLR website.

==> Sections/Truncation.tex <==




The SA procedure with truncations as described in [insert] can also be written more comprehensively. Let the step-size sequence be $\bar \bfgamma \triangleq \{ \gamma_k \}_{k \in \N_0}$, where $\gamma_k \triangleq \gamma_{k,0} = 1/(k+2)$. At each step $n\in\N_0$, let $\varsigma_n,\kappa_n$ and $\nu_n$ be \textit{counters} keeping track of the step-size index, the index of the active set, and the number of iterations since the last truncation event, respectively. With $\vx_0 \in \cK_0$, $X_0 \in \cN$ as before, and $\varsigma_0=0$, $\kappa_0=0$, and $\nu_0 = 0$, the SA procedure with truncations can be written as
%================================================
\begin{equation}\label{eqn:SA_iteration_2}
    \begin{split}
        &\text{set} ~~~~~~~\vx_{n+\frac{1}{2}} = \vx_n + \gamma_{\varsigma_n}(\bfdelta_{X_n} - \vx_n), \\
        &\text{update} ~(\vx_{n+1},\varsigma_{n+1},\kappa_{n+1},\nu_{n+1}) \\
        &~~~~~~~= 
        \begin{cases}
            (\vx_{n+\frac{1}{2}},\varsigma_{n}\!+\!1,\kappa_{n},\nu_{n}\!+\!1),~\text{if}~ \vx_{n+\frac{1}{2}} \!\in\! \cK_{\kappa_n} \!\!\!\! \\
            (\vx_{0},\varsigma_{n}\!+\!1-\!\nu_n,\kappa_{n}\!+\!1,0),~\text{otherwise}.
        \end{cases}
    \end{split}
\end{equation}
%================================================
From this point onward, we provide all our results for the iteration as shown in \eqref{eqn:SA_iteration_2}, adapting the notations therein.

Let $\mJ(\alpha)$ denote the Jacobian matrix of the right hand side of \eqref{eqn:main ode}, where $\alpha \geq 0$ is the parameter of the polynomial kernel which controls the strength of self-repellence mechanism, stemning from substituting \eqref{eqn:polynomial function} in \eqref{eqn:general srrw kernel}.
Our main theoretical results are as follows.
%================================================
\begin{theorem}[Almost sure convergence to target $\vmu$]\label{thm:first order result}
For any $\alpha \!\!\geq\!\! 0$, let $\{\vx_n\}_{n\in\N_0}$ be iterates of \eqref{eqn:SA_iteration_2}. Then, for any initial $(\vx_0,X_0) \!\in\! \cK_0 \! \times \! \cN$, the iterates $\vx_n$ converge to $\vmu$ almost surely as $n\to\infty$.
\end{theorem}


\begin{theorem}[Central Limit Theorem]\label{thm:second order result}
For any $\alpha \geq 0$, there exists $\mV(\alpha) \in \R^{N\times N}$ such that
\begin{equation}
    \sqrt{\gamma_{\varsigma_n}} (\vx_n - \vmu) \xrightarrow[dist.]{n\to \infty}N(0,\mV(\alpha)),
\end{equation}
where for all $\alpha \geq 0$,
\begin{align}
    \mV(\alpha) &= \int_0^\infty e^{t\left( \mJ(\alpha) + \eye/2 \right)}\mU {e^{t\left( \mJ(\alpha) + \eye/2 \right)}}^T dt, \\
    \mU &= \sum_{k=1}^{N-1} \frac{1+\lambda_k}{1-\lambda_k} \vu_k \vu_k^T,
\end{align}
\end{theorem}
%================================================
The following result can be shown as a consequence of the above, and is related to convergence of MCMC estimators with SRRW as the random sampler.
\begin{corollary}[]
Let $g:\cN \to \R$ be any function such that $\E_{\vmu}\left[g^2 \right] < \infty$. For any $\alpha \geq 0$, we have
\begin{equation}
    \sqrt{\gamma_{\varsigma_n}} (\vg^T\vx_n - \vg^T\vmu) \xrightarrow[dist.]{n\to \infty}N(0, \vg^T\mV(\alpha)\vg),
\end{equation}
where $\vg \triangleq [g(i)]_{i \in \cN} \in \R^N$ for all $i \in \cN$. Furthermore, for any $\alpha \geq 0$ and integer $p \in \N$, there exists a constant $C_{p,\alpha} > 0$ such that
\begin{equation}
    \sqrt{\gamma_{\varsigma_n}}\left[ \E\| \vx_n - \mu \|_p \right]^\frac{1}{p} \xrightarrow{n\to \infty} C_{p,\alpha}.
\end{equation}
\end{corollary}
The exact form of $\mV(\alpha)$ provided in Theorem \ref{thm:second order result} enables us to give the following ordering result on the asymptotic covariance.
\begin{theorem}[Ordering of asymptotic covariance]\label{thm:avr ordering and bound}
For any $\alpha_1 > \alpha_2 > 0$, we have
$$\mV(\alpha_1) <_L \mV(\alpha_2) <_L \mV(0).$$
\end{theorem}

\begin{corollary}
Moreover, for any $\alpha \geq 0$ and function $g:\cN \to \R$ such that $\E_{\vmu}\left[ g^2 \right] < \infty$, we have
\begin{equation}
    \vg^T\mV(\alpha)\vg \leq \E \left[ \frac{1}{2\alpha(1 + \Lambda) + 1} \right]\vg^T\mV(0)\vg, 
\end{equation}
where $\vg \triangleq [g(i)]_{i \in \cN} \in \R^N$, and $\Lambda\in (-1,1)$ is a random variable taking values $\lambda_i$ with probability proportional to $\vg^T \vu_i$ for all $i \in \{1,\cdots,N-1\}$.
\end{corollary}

[Still need to include some explanations for the theorems]
